FINN-R: An End-to-End Deep-Learning Framework for Fast Exploration of Quantized Neural Networks

Convolutional Neural Networks have rapidly become the most successful machine learning algorithm, enabling ubiquitous machine vision and intelligent decisions on even embedded computing-systems. While the underlying arithmetic is structurally simple, compute and memory requirements are challenging. One of the promising opportunities is leveraging reduced-precision representations for inputs, activations and model parameters. The resulting scalability in performance, power efficiency and storage footprint provides interesting design compromises in exchange for a small reduction in accuracy. FPGAs are ideal for exploiting low-precision inference engines leveraging custom precisions to achieve the required numerical accuracy for a given application. In this article, we describe the second generation of the FINN framework, an end-to-end tool which enables design space exploration and automates the creation of fully customized inference engines on FPGAs. Given a neural network description, the tool optimizes for given platforms, design targets and a specific precision. We introduce formalizations of resource cost functions and performance predictions, and elaborate on the optimization algorithms. Finally, we evaluate a selection of reduced precision neural networks ranging from CIFAR-10 classifiers to YOLO-based object detection on a range of platforms including PYNQ and AWS\,F1, demonstrating new unprecedented measured throughput at 50TOp/s on AWS-F1 and 5TOp/s on embedded devices.

==> abstract.tex <==
% Abstract
Convolutional Neural Networks have become one of the most successful
universal machine learning algorithms. They play a key role in
enabling machine vision and intelligent decisions on all kinds of
devices. While their underlying arithmetic is structurally simple,
their computational complexity is enormous and comes along with
equally challenging memory demands for storing and accessing the vast
amount of model parameters associated with trained neural networks.

A feasible and promising approach to satisfy the cost and power
constraints of a wide range of application domains is the quantization
of inputs, activations and model parameters to a reduced numerical precision.
The resulting scalability in compute performance, power savings and reduced storage footprint
provides interesting design compromises in exchange for a minimal to
modest reduction in accuracy.

Field-Programmable Gate Arrays are the ideal devices for exploring and
building low-precision neural network inference engines. Customizable
down to the bit level, they allow to pick and implement precisely the
numerical accuracy required for a particular application.

In this article we describe the second generation of the FINN
tool, which provides engineers with a means to build and evaluate
fully customized implementations of inference engines for different
precisions easily.
Leveraging an internal HLS library, it generates inference engines optimized for the specified
device and associated design targets from a simple prototext description of the
network.
We detail a selection of possible target architectures, derive an
associated hardware cost function for a broad spectrum of precisions
and use it as the basis for performance predictions.
Further, we elaborate on the previously undisclosed algorithms used
to deliver the highest performance within a given resource budget. Finally, we
demonstrate the gainable benefits of reduced precision, validate the workflow and its flexibility with results
measured for a wide range of neural networks, from small
CIFAR-10 classifiers to a YOLO-based object detection on PASCAL VOC datasets, on platforms
as small as the PYNQ-Z1 and as powerful as an AWS\,F1 instance and for different precisions.
%introduce some results


==> relatedwork.tex <==

% MERGED INTO BACKGROUND


